Counting Query Answers over a DL-Lite Knowledge Base (extended version)

Counting answers to a query is an operation supported by virtually all database management systems. In this paper we focus on counting answers over a Knowledge Base (KB), which may be viewed as a database enriched with background knowledge about the domain under consideration. In particular, we place our work in the context of Ontology-Mediated Query Answering/Ontology-based Data Access (OMQA/OBDA), where the language used for the ontology is a member of the DL-Lite family and the data is a (usually virtual) set of assertions. We study the data complexity of query answering, for different members of the DL-Lite family that include number restrictions, and for variants of conjunctive queries with counting that differ with respect to their shape (connected, branching, rooted). We improve upon existing results by providing a PTIME and coNP lower bounds, and upper bounds in PTIME and LOGSPACE. For the latter case, we define a novel query rewriting technique into first-order logic with counting.

==> 5-ignore.tex <==
  %
  % \[\bigcup\limits_{\substack{
  % (\B^1,\B^2) \in \partition(\B_k), \\
  %       n = \max\limits_{B \in \B^1} \card(B),
  %     }}
%  \julienbox{Use one of the two following definitions:
%    \[\left\{
%    \begin{array}[t]{@{}l}
%        \left\langle\
%    \begin{array}[t]{@{}l}
%      qh(n{-}i), \{\rpl(r, \atDec(\B^3, \B^2) \land \exists^{=i}_y R(x,y)) \\
%      \hspace{2.5cm} \mid{} \B^3 \in \comb_\T(\B^1), r \in \Pi'\}\\
%    \end{array}
%  \right\rangle\\
%      \hspace{0.2cm}\mid{}
%       (\B^1,\B^2) \in \partition(\B_k), 
%        n = \max\limits_{B \in \B^1} \card(B),\\
%      \hspace{0.4cm}i \in [0 .. n-1] 
%    \end{array}
%\right\}
% \]
% }


\begin{proposition} \dllitecoreNmin has a universal model w.r.t.\
  \countP over \CQCR queries.
  \end{proposition}
  \begin{proof}[Proof (sketch).]
    We show that the restricted chase is a universal model,
    by induction on the number of atoms in the query. The %induction \
    base case can be proved by induction,
    over the number of chase steps,
    %which
    comparing the sets
    of matches for the (atomic and rooted) query in the interpretations
    $\inter(\chase_{j}(\K))$ and $\inter(\chase_{j+1}(\K))$.

    For the inductive step,
      we use the model $\C := \inter(\chase_\infty(\K))$,
      and we analyze the sets $\Omega^i_\C$ and
      $\Omega^{i+1}_\C$ that contain respectively 
    the matches in $\C$ for the subqueries composed of the $i$ and $i$+1 first atoms of the input query $q$.
    
    We proceed by case analysis on of the $i$-th atom,
    and assume by contradiction that there exists a model $\I$
    such that $|\Omega^{i+1}_\I| < |\Omega^{i+1}_\C|$. 
    To derive the contradiction
    we exploit the properties of a generic homomorphism from $\C$ to $\I$,
    which always exists due to the fact that $\C$ is a canonical model.
\end{proof}


% \davidebox{Remove notion of position}
%Given a term $t = f(t_1, \ldots, t_n)$, the \emph{subterm of $t$ at position $p$}, denoted as $t|_p$, is defined as $t$ if $p=\varepsilon$, and as $t_i|_q$ if $p=iq$.
%\davidebox{TODO: It is not really necessary to define positions over terms. CHANGE.}
%Such notion extends to atoms and conjunction of atoms in the natural way.

% Given a conjunction of atoms $\psi = X(\t_1), \land \ldots, \land X(\t_n)$, we denote by by $\psi[\phi]_p$ the expression obtained by replacing the element at position $p$ with the formula $\phi$.
% To represent deletion, we denote by $\psi[\varepsilon]_p$ the formula obtained by
% removing the element in position $p$ from $\psi$. To denote $n$ concurrent replacements or removals at positions $p_1,\ldots,p_n$, we use the notation $\psi[\alpha_1, \ldots, \alpha_n]_{p_1,\ldots,p_n}$. Note that this is not the same as applying the unary replacement operation $n$ times.
% % If the $\alpha_1, \ldots \alpha_n$ are all the same $\alpha$, then we will use the short notation $\psi[\alpha]_{p_1,\ldots,p_n}$.

\davidebox{I have put-back the restriction on the unifiers, so that given an atom $R(x,y)$:
  \begin{itemize}
  \item If I have renamed $y$ (into some other aggregation variable), then $y$ is blocked and therefore no gealpha.
  \item I try to not invent new names for variables (and also not to bind what was unbound)
  \end{itemize}
}

\davidebox{Was:
    
    $\bigcup\limits_{\substack{(\B^1,\B^2) \in \partition(\B_k), \\
        n = \max_{B \in \B^1} \card(B),\\ i \in [0 .. n-1]
      }}
    \begin{array}[t]{@{}l}
      \hspace{-9mm}\{\tup{\qh(n{-}i), \rpl(r, \atDec(\B^3, \B^2) \land \exists^{=i}_y R(x,y))} \mid{}\\
      \hspace{3.3cm} \B^3 \in \comb_\T(\B^1)\}
    \end{array}$
  }
   \julienbox{
     Seems like the  older version was equivalent to:
     $\bigcup\limits_{\substack{(\B^1,\B^2) \in \partition(\B_k), \\
         n = \max_{B \in \B^1} \card(B),\\ i \in [0 .. n-1],\\
         \B^3 \in \comb_\T(\B^1)
       }}
     \begin{array}[t]{@{}l}
       \hspace{-9mm}\{\tup{\qh(n{-}i), \{\rpl(r, \atDec(\B^3, \B^2) \land \exists^{=i}_y R(x,y))}\} \\
     \end{array}$
   }
   \julienbox{
     Now I guess it should be as follows:
     $\bigcup\limits_{\substack{(\B^1,\B^2) \in \partition(\B_k), \\
         n = \max_{B \in \B^1} \card(B),\\ i \in [0 .. n-1]}
       }
     \begin{array}[t]{@{}l}
       \hspace{-9mm}\{\tup{\qh(n{-}i), \{\rpl(r, \atDec(\B^3, \B^2) \land \exists^{=i}_y R(x,y)) \mid{} \\
        \hspace{3.3cm} \B^3 \in \comb_\T(\B^1)\}}\}
     \end{array}$
     \davidebox{Looks like you are right. However now, since application of gealpha must occur in parallel, observe that now I added a $\Pi'$ in the formula. I think my version is more readable, although yours might be shorter: I find putting all conditions under the union a bit confusing.}
     \julienbox{
       I guess we don't read the same way :)\\
       For me it is significanlty more difficult to have nested expressions,
       because I need to carefully check where the nested parentheses or brackets  open and close.
     }
   }

\davidebox{TODO: Define $\y \setminus_{pos} pos(y,\s)$ (Meaning: $pos(y,\s)$ = position(s) of $y$ in $\s$. By $\setminus_{pos}$, we say that want to remove from $\y$ the variable at position(s) $pos(y,\s)$.
  \davidebox{I have removed it. First, $y$ cannot be renamed or if it is then gealpha and gebeta are blocked anyways. Second, I want to leave all details about renamings out.}
}

\julienbox{
    Check whether it is all atoms or all $\exists$-atoms
.  }
  %from $\body(\rpl(r,\phi))$.

  % with the additional condition that rule $r'$ is such that all $\exists$-atoms in which variable $w$ occurs are removed.
%  \rdef \bigvee_\varphi \psi^\kappa[\phi,\bm{\varepsilon}]_{p,\bm{p}}\}$, where positions $\bm{p}$ are all positions other than $p$ of the atoms in which $y$ occurs.
  % \julienbox{
    % If we choose to follow the alternative presentation of $\gealpha$ above, then this becomes:\\
    
  % }

\davide{Given a pair $\tup{Q(\y, \aggCount(\y) \cdot \alpha, \Pi}$ and a rule
$r \in \Pi$, we denote by $\normrule{Q}(r)$, which we call \emph{the normalized
form of $r$ w.r.t.\ $Q$}, obtained by renaming the variables in $r$, based on their
positions, according to $\x$ and $\y$, and by replacing constants and repeated
variables in the head of $r$ with suitable equalities in its body. Similarly, we
extend the notion to an atom $R(x,y)$ through the notation
$\normatom{Q}{r}(R(x,y))$. We indicate the inverse operations through the notation
$\normrule{Q}^{-1}(r')$ and $\normatom{Q}{r}^{-1}(R(x',y'))$, respectively.}
\davidebox{For sure, TO BE REFINED. Maybe an example?}

\julienbox{[Davide> TODO]
  This proof sketch is a little bit cryptic.
 We may either:
  \begin{itemize}
  \item make it more high-level (e.g. no need to say that that we proceed by contradiction or by case analysis if we do not povide the actual proof)
 \item provide more details (uncomment the end)
   \end{itemize}
   \davidebox{I think it is not cryptic, however if you have a proposal for making it more high-level please go ahead.}
 }

  
  \begin{lemma}
    \label{lemma:core-property} Given a \dllitecoreNMINUS KB $\K$, a
role name $P$ and an individual $o \in \NI \cup \NE$, if $\inter(\chase_{\infty}(\K)) \models (\ge n P)(o)$ then for every interpretation $\I$ model of $\K$, for every homomorphism $\tau$ from $\inter(\chase_{\infty}(\K)$) to $\I$, it holds that $\I \models (\ge n P)(\tau(o))$.
\begin{proof}[Proof (sketch).]
  By construction of the \emph{restricted} chase.
\end{proof}
\end{lemma}
%
Lemma~\ref{lemma:core-property} holds only if we forbid the generalization of roles occurring in the RHS of a
concept inclusion. \dlliter plus this restriction corresponds to the logic \dlliterminusb \cite{NKKK*19}, which in fact is BCALC-rewritable for \CQR{}s.

% <<<<<<< HEAD We now detail the four rewriting rules of \perfectrefcount. We use the
% symbol underscore '$\_$' to denote the fresh variables that are introduced during
% the execution of the algorithm. Given a basic concept $B$, the function application
% $\xi(B,x)$ returns $B(x)$ if $B \in \NC$, or $R(x,\_)$, if $B = \GEQ{1}{R}$. Given
% a set $N$ of basic concepts, $\sat_\T(N)$ is defined as the set
% $\setB{B'}{B' \sqsubseteq_\T B, B \in N}$.  If $\phi, \psi$ are two formulae and
% $a$ an atom, we use $\phi[a/\psi]$ (resp. $\phi[a/\top]$) to designate the formula
% identical to $\phi$, but where $a$ is replaced with $\psi$ (resp. where $a$ is
% deleted from $\phi$).  By extension, if $r$ is a rule, we use $r[a/\psi]$ to
% designate the rule $\head(r) \rdef \body(r)[a/\psi]$.  \davidebox{Use macro GEQ
% everywhere!!}  =======

% For technical reasons we assume that $\T$ does \emph{not} contain existential restrictions of the form $\exists R$ on the RHS of axioms, and only allows for the equivalent %(but syntactically different) form $\ge 1 R$.
%   %
$\rdef (\bigvee_{i=1}^n \psi^i) \lor \sigma(\psi^j)[\phi,\varepsilon]_{p_1,p_2}$, where $\phi = X(\sigma(\z_1)) \land \tau(\z_1 = \sigma(\z_1) \land \z_2 = \sigma(\z_2))$
%   %\davide{and $\tau$ is a function that removes repeated or trivial (i.e., $x=x$) equalities and all those equalities involving variables that were introduced during the execution of the algorithm (i.e., that were not part of the original query). TODO: REMOVE TAU, not needed.}
% \julienbox{
%     In the definition of $\tau$, I would drop the mention of trivial or repeated inequalities (makes the definiton unnecessarily heavy), and keep only the elimination of variables that were introduced during the execution.\\
%     I.e. I would avoid mentioning ``syntactic cleaning'' in the formal definition.\\
%     I proposed yesterday to remove trivial equalities from the examples, because at first sight they may look like typos.\\
%     I think we can drop them without explanation.
%     Or if you want, write in the example ``we dropped trivial equalities of the form $x = x$ here, for readability''.
% }

\begin{table*}
  \caption{\davidebox{TODO: Define $\y \setminus_{\mathsf{p}} \pos(y,\s)$ (Meaning: $\pos(y,\s)$ = position(s) of $y$ in $\s$. By $\setminus_{\mathsf{p}}$, we say that want to remove from $\y$ the variable at position(s) $\pos(y,\s)$. By $r[q(\s,\t) / q(\s,\t \setminus \{y\})$, I mean that we replace $q(\s,\t)$ in $r$ with $q(\s,\t \setminus \{y\})$. adec is ``Atomic decomposition''}
  }
  \begin{tabular}{l}
    $\bigcup_{\begin{array}{ll}
                N \subseteq \B, N \neq \emptyset, M = \B \setminus N, \\
                \sat_\T(N) \cap \sat_\T(M) = \emptyset, \\
                n_{\max} = \max\{n_j\ |\ B_j \in N\}, \\
                i \in \{0, \ldots, n_{\max}\}
              \end{array}} \begin{array}{l}
                             \{ Q(q(\x, \aggCount(\y \setminus_{pos} pos(y,\s)) \cdot (n_{\max} - i) \cdot \alpha_k), \\ 
                             \setB{r[q(\s,\t) / q(\s,\t \setminus \{y\}), R(x,y)/adec(N',M)] \land \exists^{=i}y R(x,y)]}{N' \in \comb(N,\T)})\}
                           \end{array}$
  \end{tabular}
\end{table*}

\myparagraph{\gealpha ($\rightsquigarrow_{\ge_\alpha}$).} $\{\mathfrak{q}_1, \ldots, \mathfrak{q}_k\} \rightsquigarrow_{\ge_\alpha} \{\mathfrak{q}_1, \ldots, \mathfrak{q}_k\} \cup \Q_k$ if
%
\begin{compactitem}
\item $\mathfrak{q}_k = \tup{Q(\x, \aggCount(\y) \cdot \alpha), \Pi}$ % $\rdef \bigvee_{\gamma=1}^\delta \psi^\gamma$;
  % \item[$\star$] $\psi^\kappa|_p = R(x,y)$ with $y$ unbound, for some $\kappa \in \{1,\ldots,\delta\}$;
\item[$\star$] $R(x,y) \in \body(r)$ with $y$ non-blocked, for some $r \in \Pi_k$;
\item $\head(r) = q(\s,\t)$, for tuples of terms $\s$ and $\t$ such that $y \in \t$.
\item $\{B_1 \sqsubseteq\ \ \ge_{n_1} R, \ldots, B_\ell \sqsubseteq\ \ \ge_{n_\ell} R\} \subseteq \T$;
\item[$\diamond$] $\Q_k = \bigcup_{\S} \{ Q(q(\x, \aggCount(\y \setminus_{pos} pos(y,\s)) \cdot n' \cdot \alpha_k), \Pi_k')\}$.
%\item[$\diamond$] $\Q_k = \bigcup_{\S} \{ Q_k'(q(\x, \aggCount(\y') \cdot n'), \Pi_k') \rdef \bigvee_\varphi \psi^\kappa[\phi]_p \}$.
\end{compactitem}
%
Condition $\S$, multiplicative factor $n'$ and set $\Pi'$ of rules in item $\diamond$ are defined as follows.
Let $\B := \{B_1, \ldots, B_\ell\}$. Then $\S$ is the set of conditions $\{N \subseteq \B, N \neq \emptyset, M = \B \setminus N, \sat_\T(N) \cap \sat_\T(M) = \emptyset, n_{\max} = \max\{n_j\ |\ B_j \in N\}, i \in \{0, \ldots, n_{\max}\}\}$. The symbol $n'$ stands for the expression $(n_{\max} - i)$. \julien{\st{If $N = \{B_{N_1}, \ldots, B_{N_k}\}$, then }}the set $\Pi'_k$ of rules is $\setB{r'}{N' \in \comb_\T(N)}$,
where \julien{\st{$\comb(N,\T) = \setB{\{B_{N_1}', \ldots, B_{N_k}'\}}{B_{N_i}' \in \sat_\T(\{ B_{N_i}\}), 1 \le i \le k}$}
  $\comb_\T(N)$ is the cartesian product $\prod\limits_{B \in N} \sat_\T(B)$
}
  , and $r'$ is a copy of rule $r$ in which the atom $R(x,y)$ is replaced by the following \emph{atomic decomposition formula}:
%
\[\bigwedge_{B \in N'} \!\!\! \xi(B,x)
  \land \bigwedge_{B \in M,B' \sqsubseteq_\T B} \!\!\! \!\!
  \lnot \xi(B',x) \land \exists^{=i}_y R(x,y)\]
%
and such that $\head(r') = q(\s,(\t \setminus \{y\}))$.
\davidebox{Maybe denote range as $[1..4]$.} 


\[\left\{\hspace{-.1cm}\begin{array}{l@{\hspace{1ex}}l@{\hspace{1ex}}l}
                      \tup{Q(x,\aggCount(y,z) \cdot 1), \{q(x : y,z) \\
                      & \hspace{-1cm} \rdef A(x), R_1(x,y), R_2(y,z)\}},\\
                      \tup{Q(x, \aggCount(y) \cdot 3 - 0),\{q(x : y)\\
                      & \hspace{-1cm} \rdef A(x), R_1(x,y), \\
                      & \hspace{-.6cm} R_1(w_1,y), \exists^{=0}_z R_2(y,z)\}},\\
                      \tup{Q(x, \aggCount(y) \cdot 3 - 1), \{q(x : y) \\
                      & \hspace{-1cm} \rdef A(x), R_1(x,y), \\
                      & \hspace{-.6cm} R_1(w_1,y), \exists^{=1}_z R_2(y,z)\}},\\
                      \tup{Q(x, \aggCount(y) \cdot 3 - 2), \{q(x : y) \\
                      & \hspace{-1cm} \rdef A(x), R_1(x,y), \\
                      & \hspace{-.6cm} R_1(w_1,y), \exists^{=2}_z R_2(y,z)\}}\\
                    \end{array}\hspace{-.1cm}\right\}
                \]

\julienbox{
  Can we stick to the notation $i,j \in \{1, .., n\}$ for indices (as previously),
  instead of $\kappa,\delta \in \{1, .., \gamma\}$?\\
  Also what is $i$ in $(n_{\max} - i)$?
  \davidebox{
    As you see, I have finished the letters for indexes. If you think you can implement this quickly, consistently, (also with ge\_beta), and without mixing the indexes (and I am sure that under rush I can make a mistake for each of these categories) please go ahead.
    The number $i$ is defined in $\S$.
  }
  \julienbox{
    Ok, so if $i$ (used in $(n_{\max} - i)$) refers to something that appears only in the definition of $\S$, then this becomes really hard to parse.\\
    Maybe we could adopt a bottom up definition instead.
    E.g.
    \begin{itemize}
    \item first define explicitly the function ``atomDecomp($N$)'' (or maybe ``atomDecomp($\B$)'') that takes (a family of) sets of concepts, and returns the formula ...
      \item then only define $\Q_k$, using  ``atomDecomp()''. 
    \end{itemize}
    As for the indices, by decomposing the definitions in this fashion, hopefully we will be able to use $i, j$ and $k$ everywhere, with local scope, and without ambiguity.
    \davidebox{Ok, I will try to do this}.
  }
}

\julienbox{
  Can we stick to the notation $i,j \in \{1, .., n\}$ for indices (as previously),
  instead of $\kappa,\delta \in \{1, .., \gamma\}$?\\
  Also what is $i$ in $(n_{\max} - i)$?
  \davidebox{
    As you see, I have finished the letters for indexes. If you think you can implement this quickly, consistently, (also with ge\_beta), and without mixing the indexes (and I am sure that under rush I can make a mistake for each of these categories) please go ahead.
    The number $i$ is defined in $\S$.
  }
  \julienbox{
    Ok, so if $i$ (used in $(n_{\max} - i)$) refers to something that appears only in the definition of $\S$, then this becomes really hard to parse.\\
    Maybe we could adopt a bottom up definition instead.
    E.g.
    \begin{itemize}
    \item first define explicitly the function ``atomDecomp($N$)'' (or maybe ``atomDecomp($\B$)'') that takes (a family of) sets of concepts, and returns the formula ...
      \item then only define $\Q_k$, using  ``atomDecomp()''. 
    \end{itemize}
    As for the indices, by decomposing the definitions in this fashion, hopefully we will be able to use $i, j$ and $k$ everywhere, with local scope, and without ambiguity.
    \davidebox{Ok, I will try to do this}.
  }
}

\julienbox{
  Can we stick to the notation $i,j \in \{1, .., n\}$ for indices (as previously),
  instead of $\kappa,\delta \in \{1, .., \gamma\}$?\\
  Also what is $i$ in $(n_{\max} - i)$?
  \davidebox{
    As you see, I have finished the letters for indexes. If you think you can implement this quickly, consistently, (also with ge\_beta), and without mixing the indexes (and I am sure that under rush I can make a mistake for each of these categories) please go ahead.
    The number $i$ is defined in $\S$.
  }
  \julienbox{
    Ok, so if $i$ (used in $(n_{\max} - i)$) refers to something that appears only in the definition of $\S$, then this becomes really hard to parse.\\
    Maybe we could adopt a bottom up definition instead.
    E.g.
    \begin{itemize}
    \item first define explicitly the function ``atomDecomp($N$)'' (or maybe ``atomDecomp($\B$)'') that takes (a family of) sets of concepts, and returns the formula ...
      \item then only define $\Q_k$, using  ``atomDecomp()''. 
    \end{itemize}
    As for the indices, by decomposing the definitions in this fashion, hopefully we will be able to use $i, j$ and $k$ everywhere, with local scope, and without ambiguity.
    \davidebox{Ok, I will try to do this}.
  }
}

\julienbox{
  Can we stick to the notation $i,j \in \{1, .., n\}$ for indices (as previously),
  instead of $\kappa,\delta \in \{1, .., \gamma\}$?\\
  Also what is $i$ in $(n_{\max} - i)$?
  \davidebox{
    As you see, I have finished the letters for indexes. If you think you can implement this quickly, consistently, (also with ge\_beta), and without mixing the indexes (and I am sure that under rush I can make a mistake for each of these categories) please go ahead.
    The number $i$ is defined in $\S$.
  }
  \julienbox{
    Ok, so if $i$ (used in $(n_{\max} - i)$) refers to something that appears only in the definition of $\S$, then this becomes really hard to parse.\\
    Maybe we could adopt a bottom up definition instead.
    E.g.
    \begin{itemize}
    \item first define explicitly the function ``atomDecomp($N$)'' (or maybe ``atomDecomp($\B$)'') that takes (a family of) sets of concepts, and returns the formula ...
      \item then only define $\Q_k$, using  ``atomDecomp()''. 
    \end{itemize}
    As for the indices, by decomposing the definitions in this fashion, hopefully we will be able to use $i, j$ and $k$ everywhere, with local scope, and without ambiguity.
    \davidebox{Ok, I will try to do this}.
  }
}

Conditions $\S$, $\varphi$, formula $\phi$, and $n'$ in bullet $\diamond$ are defined as follows. Let $\B := \{B_1, \ldots, B_\ell\}$. Then
$\S$ is the set of conditions $\{N \subseteq \B, N \neq \emptyset, M = \B
\setminus N, \sat_\T(N) \cap \sat_\T(M) = \emptyset, n_{\max} =
\max\{n_j\ |\ B_j \in N\}, i = \{0, \ldots, n_{\max}\}\}$, where
$\sat_\T$ is a function taking a set of concepts $B$ and returning the set of all concepts $B'$ such that $B' \sqsubseteq_\T B$. If $N = \{B_{N_1}, \ldots, B_{N_k}\}$, then the condition $\varphi$ is the expression $N' \in \setB{\{B_{N_1}', \ldots, B_{N_k}'\}}{B_{N_i}' \sqsubseteq_\T B_{N_i}, 1 \le i \le k}$. $n'$ is the expression $(n_{\max} - i)$.
Formula $\phi$, that we call \emph{atomic decomposition}, is then defined as:
%
\[\bigwedge_{B \in N'} \!\!\! \xi(B,x)
  \land \bigwedge_{B \in M,B' \sqsubseteq_\T B} \!\!\! \!\!
  \lnot \xi(B',x) \land \exists^{=i}y R(x,y)\]
%
where function $\xi$ is defined as for \atomrewrite.
\davidebox{TODO: Consider renaming variable $y$!! This would leave spurious equalities, but not a huge issue.}

% The restrictions on the unifier are meant to preserve, through the use of equality atoms, the head of query $q$.
% \julienbox{
%   I think what you mean is:\\
%   ``$\phi$ is the formula $X(\sigma(\z_1)) \land \z_1 = \sigma(\z_1) \land \z_2 = \sigma(\z_2)$''\\
%  As it is currently written, it is not immediately clear whether the ``='' symbols are inside the defintion or not, i.e. whether you define
%  just $\phi$, or instead $\phi$, $z_1$ and $z_2$.
%  \davidebox{Ok, changed here. Need to see whether I can change everywhere without losing too much space.}
% }
% \julienbox{
%   Confused by the Reduce rule, because it seems that the query that is poduced is equivalent to the input one.\\
%   Precisely, seems like the subquery $\sigma(\psi^j)[\phi,\varepsilon]_{p_1,p_2}$ is contained in the subquery $\psi^j$.\\
%   Maybe I am missing something that pertains to cardinalities?
%   \davidebox{
%     Why do you say subqueries?
%     \julien{I mean ``subformula'' in the final rewriting.}
%     Imagine $P(x,y) \land P(\_,x)$. If I apply reduce, then I get $P(x,x) \land x=\_ \land y=x \land \_=x \land  x=x$ (yeah, many repetitions.. this could be improved), which is not a subquery.

%     \julienbox{
%       According to the definition of Reduce, in this example, you get a \textbf{disjunction} of two CQs.
%       The first one is $\psi^j$ (i.e. in this example $P(x,y) \land P(\_,x)$) and the second one is $\sigma(\psi^j)[\phi,\varepsilon]_{p_1,p_2}$ (i.e. in this example  $P(x,x) \land x=\_ \land y=x \land \_=x \land  x=x$).\\
%       My concern is that $\sigma(\psi^j)[\phi,\varepsilon]_{p_1,p_2}$ is contained (in the sense of query containment) in $\psi^j$.\\
%       For instance, in the running example (next page), the first disjunct seems ``redundant'' or ``unnecessary''.
%       \davidebox{As I said in the example, the reduce step creates sub-queries which have less bound variables, so that you are then able to
%         apply more rewriting rules. The same happens with the normal Perfectref.
%       }
%     }
    
%     The goal of reduce is to render
%     certain variables unbound, so as to be able perform the other rewriting rules afterwards (otherwise these rules would be blocked, because
%     they require an unbound variable). Note that we do not consider variables occurring in equality (or negated) atoms as bounded. The technical reason
%     is that these ``special atoms'' are never considered as target atoms for the application of a rule (and therefore we do not care whether their variables
%     are bounded or not). The fact that this ``ignoring'' is sound should be guaranteed by the equalities. The equalities also allow us not to apply the unifier in the head.
%   }
% }
% \davidebox{Question: is $\sqsubseteq_\T$ defined?\\
%   \julien{If you mean concept entailement wrt $\T$,
%     the answer is no.\\
%     But I can do it informally in the preliminaries.
%   }
%   \davidebox{
%     Please go ahead. 
%   }
% }
%

Summing up, our target language allows for queries of the kind

\[q(\x, \aggCount(\y) \cdot \alpha) \rdef \psi^1 \vee .. \vee \psi^n\]

where each  $\psi^i$ is of the form:

\[\psi^k_{pos} \land \psi^k_{neg} \land \psi^k_{eq} \land \psi^k_{\exists}\]

In $q$, $\x$ are the distinguished variables, $\aggCount(\y)$ (intuitively
corresponding to the SQL construct \textsc{count distinct}) specifies the
aggregation variables $\y$, all variables in $\x,\y$ occur in the body of $q$, $\x \cap \y = \emptyset$, $\alpha \in \mathbb{N}$ is a positive
multiplicative factor, $\psi_{pos}$ is a conjunction of positive atoms, $\psi_{neg}$ is a conjunction of negated atoms, $\psi_{eq}$ is a conjunction of equalities between terms, and $\psi_{\exists}$ is a conjunction

\[\bigwedge_{i=1}^n \exists^{=j_i} y_i P_i(x_i,y_i)\text{, where each
$j_i$} \in \mathbb{N}_0\]

where each variable $y_i$ occurs only in the atom $P(x_i,y_i)$.
We call each expression $\exists^{=j_i} y_i P_i(x_i,y_i)$ an $\exists$-atom.

A mapping $\rho$ is a match for $\psi^k$ in an interpretation $\I$ if:
\begin{compactitem}
\item $\rho(\psi^k_{pos}) \subseteq \I$,
\item $\rho$ satisfies all equalities in $\psi^k_{eq}$,
%\item $\lnot\exists \rho' \supseteq \rho : \rho'(\psi_{neg}) \cap \I \neq \emptyset$,}
\item there is no $\rho' \supseteq \rho$ s.t.  $\rho'(\psi^k_{neg}) \cap \I \neq \emptyset$
  
\item there exist \emph{exactly} $j_i$ mappings $\rho''$ such that:
  \begin{compactitem}
  \item $\rho'' \supseteq \rho$ and
  % \item $\forall i : \rho''(P(x_i,y_i)) \subseteq \I$.
  \item for all $i$, $\rho''(P(x_i,y_i)) \subseteq \I$.
  \end{compactitem}
\end{compactitem}
%
A mapping $\rho$ is a match for $q$ if it is a match for some $\psi^i$ occurring in the body of $q$.
A mapping $\omega$ is an \emph{answer} to $q$ over $\I$ with cardinality $k
\cdot \alpha$ iff there are \emph{exactly} $k$ mappings $\eta_1, \ldots, \eta_k$ such that:
%
\begin{compactitem}
\item $\omega = \eta_i|_{\x}$, for each $i \in \{1,\ldots, k\}$, and
\item each $\eta_i$ can be extended to a match $\rho$ for $q$ in $\I$ such that $\rho|_{\x \cup \y} = \eta_i$. 
\end{compactitem}


Note that our semantics also captures the case when the operator $\aggCount()$ is over an empty set of variables (in that case, the $k$ above would be equal to $1$). This technicality is necessary for the presentation of the algorithm. 

From now on, we also say that a variable $x$ in a query $q$ is \emph{bound} if it is a distinguished variable or it occurs more than once in $\psi_{pos} \land \psi_{\exists}$.

==> garbage.tex <==


\subsection{Proposition~\ref{prop:hardness_branching}}

  \textsc{Count} is \coNP-hard in data complexity for \dlliteposH and acyclic,
  connected, but branching CQs (\CQAC).

 \begin{proof}
   Again, we adapt the reduction from (co-)3-colorability from~\cite{KoRe15},
so that the Gaifman graph of the query used in the reduction is acyclic,
 and has a single connected component.\\
 Let $G = \tup{V, E}$ be an undirected graph without self-loop (with vertices $V$ and edges $E$).\\
 We define the KB $\K = \tup{\T,\A}$ as follows.
    \begin{itemize}
    \item $\A = \A_1 \cup \A_2 \cup \A_3 \cup \A_4 \cup \A_5$, where:
    \begin{itemize}
     \item 
       $\A_1 = \{\ex{Vertex}(v)\mid v \in V\} \cup \{\ex{edge}(v_1, v_2)\mid (v_1, v_2) \in E\}$
     \item
       $\A_2= \{\ex{conn}(v_1,v_2)\mid v_1, v_2 \in V\}$
   \item
     $\A_3 = \{\ex{s}(v,c) \mid v \in V \text{ and } c \in \{\ex{b, g, r}\}\}$
   \item  
     $\A_4 = \{\ex{edge}(\ex{a, a}), \ex{conn}(\ex{a,a}), \ex{hasColor}(\ex{a, b}), \ex{hasColor}(\ex{a, g}), \ex{hasColor}(\ex{a, r})\}$
   \item
     $\A_5 = \{\ex{Blue}(\ex{b}), \ex{Green}(\ex{g}), \ex{Red}(\ex{r})\}$
     \end{itemize}
   \item $\T = \T_1 \cup \T_2$, where:
     \begin{itemize}
     \item 
       $\T_1 = \{\ex{Vertex} \sqsubseteq \exists \ex{hasColor}\}$
     \item $\T_2 = \{\ex{s} \sqsubseteq \ex{u}, \ex{hasColor} \sqsubseteq \ex{u}\}$
   \end{itemize}
 \end{itemize}
 \noindent Observe that the KB $\K = \tup{\T,\A}$ is satisfiable.\\
 
 \noindent We now define the query $q$ as: 
$$q() \rdef \phi_b \wedge \phi_g \wedge \phi_r  \wedge \phi_1  \wedge \phi_2$$
where:
    \begin{itemize}
    \item $\phi_b = \ex{edge}(v_1, v_2) \wedge \ex{hasColor}(v_1, c_1) \wedge \ex{hasColor}(v_2, c_2) \wedge \ex{Blue}(c_1) \wedge \ex{Blue}(c_2)$
    \item $\phi_g = \ex{edge}(v_3, v_4) \wedge \ex{hasColor}(v_3, c_3) \wedge \ex{hasColor}(v_4, c_4) \wedge \ex{Green}(c_3) \wedge \ex{Green}(c_4)$
    \item $\phi_r = \ex{edge}(v_5, v_6) \wedge \ex{hasColor}(v_5, c_6) \wedge \ex{hasColor}(v_6, c_6) \wedge \ex{Red}(c_5) \wedge \ex{Red}(c_6)$
    \item $\phi_1 = \ex{conn}(v_1, v_3) \wedge \ex{conn}(v_3, v_5)$   
    \item $\phi_2 = \ex{s}(v_7, c_1) \wedge \ex{u}(v_7, c_7)$ 
    \end{itemize}
  Observe that the Gaifman graph of $q$ is a tree.\\
  % Observe also that $c_1$ is the only variable shared by $\phi_b$ and $\phi_2$.\\


  We now show that $\certCard(q,\K) \geq 3 \cdot |V| + 1$ iff $G$ is not 3-colorable.
   \begin{itemize}
    \item $(\Rightarrow)$
      By contraposition.\\
      Let $G$ be 3-colorable.\\
     We show that there is a model $\I$ of $\K$ such that $\tup{\varepsilon, 3 \cdot |V|} \in \ans(q,\I)$.\\
      It follows that $\certCard(q,\K) < 3 \cdot |V| + 1$.\\
      
    \noindent $\I$ is defined as follows:
      \begin{itemize}
      \item for $E \in \{\ex{Vertex, edge, hasColor, s, conn, Blue, Green, Red}\}$,
      $E^\I = E^{\A}$,
     \item $\ex{u}^\I = \ex{hasColor}^\I \cup \ex{s}^\I$,
    \item 
      each $v \in (\ex{Vertex}^\I)$ has a unique \ex{hasColor}-successor,
      among $\ex{\{b, g, r\}}$,
       such that no adjacent vertices have the same successor;
       this is possible since $G$ is 3-colorable (by assumption).
      \end{itemize}
    It can be verified that $\I$ is a model of $\K$.\\

    
    Then
    $\phi_b^\I = \{\{
     v_1 \mapsto \ex{a},
     v_2 \mapsto \ex{a},
     c_1 \mapsto \ex{b},
     c_2 \mapsto \ex{b}
     \}\}$,
    and similarly for $\phi_g^\I$ and $\phi_r^\I$ (with $\ex{g}$ and $\ex{r}$ respectively instead of $\ex{b}$).\\
    Therefore $|\phi_b^\I| = 1$ (and similarly for $\phi_g^\I$ and $\phi_r^\I$).\\
      In addition,
    $\{
     v_1 \mapsto \ex{a},
     v_3 \mapsto \ex{a},
     v_5 \mapsto \ex{a}
     \}
     \in \phi_1^\I$.\\
     So $(\phi_b \wedge \phi_g \wedge \phi_r \wedge \phi_1)^\I =$
     \[
       \left\{
       \begin{array}{llll}
     v_1 \mapsto \ex{a},& v_2 \mapsto \ex{a},& c_1 \mapsto \ex{b},& c_2 \mapsto \ex{b},\\
     v_3 \mapsto \ex{a},& v_4 \mapsto \ex{a},& c_3 \mapsto \ex{g},& c_4 \mapsto \ex{g},\\
     v_5 \mapsto \ex{a},& v_6 \mapsto \ex{a},& c_5 \mapsto \ex{r},& c_6 \mapsto \ex{r}
       \end{array}
       \right\}
     \]
     
Finally,
$\phi_2[c_1/\ex{b}]^{\I} =  \{ \{v_7 \mapsto v, c_7 \mapsto c\} \mid v \in V, c \in \{\ex{b,g,r}\}\}$.\\
So $|\phi_2[c_1/\ex{b}]^{\I}| = 3 \cdot |V|$.\\ 
  % \mid \mapsto\}V \times \{\ex{r}\}$ 
% We said that $|\phi_1^{\I}| = 1$, and in particular the unique assignment sets $c_1 = \ex{r}$. \\
      % Then , $\phi_2[(c_1)/(\ex{r})]^{\I} = V \times \{\ex{b, g, r}\}$,\\
Therefore $|(\phi_b \wedge \phi_g \wedge \phi_r  \wedge \phi_1  \wedge \phi_2)^\I | = 1 \cdot 3 \cdot |V| = 3 \cdot |V|$.\\
It follows that $\tup{\varepsilon, 3 \cdot |V|} \in \ans(q,\I)$.


   \item $(\Leftarrow)$
     Let $G$ be non 3-colorable.\\
    We show below that for any model $\I$ of $\K$,
    there is a $k_\I \ge 3 \cdot |V| + 1$ s.t. $\ans(q,\I) = \{\tup{\varepsilon, k_\I}\}$.\\
    It follows that $\certCard(q,\K) \geq 4$.\\

     Let $\I$ be a model of $\tup{\T, \A}$.\\
     Then
    $\{
     v_1 \mapsto \ex{a},
     v_2 \mapsto \ex{a},
     c_1 \mapsto \ex{b},
     c_2 \mapsto \ex{b}
     \}\in \phi_b^\I$,
    and similarly for $\phi_g^\I$ and $\phi_r^\I$ (with $\ex{g}$ and $\ex{r}$ respectively instead of $\ex{b}$).\\

      In addition,
    $\{
     v_1 \mapsto \ex{a},
     v_3 \mapsto \ex{a},
     v_5 \mapsto \ex{a}
     \}
     \in \phi_1^\I$.\\
     So 
     \[
       \left\{
       \begin{array}{llll}
     v_1 \mapsto \ex{a},& v_2 \mapsto \ex{a},& c_1 \mapsto \ex{b},& c_2 \mapsto \ex{b},\\
     v_3 \mapsto \ex{a},& v_4 \mapsto \ex{a},& c_3 \mapsto \ex{g},& c_4 \mapsto \ex{g},\\
     v_5 \mapsto \ex{a},& v_6 \mapsto \ex{a},& c_5 \mapsto \ex{r},& c_6 \mapsto \ex{r}
       \end{array}
     \right\}
     \in (\phi_b \wedge \phi_g  \wedge \phi_r \wedge \phi_1)^\I
     \]

     
     Now let $\Omega = \{ \{v_7 \mapsto v, c_7 \mapsto c\} \mid v \in V, c \in \{\ex{b,g,r}\}\}$.\\
     Because $\A_3 \subseteq \I$ and $(\ex{s} \sqsubseteq \ex{u}) \in \T$,
     it must be the case that $\Omega \subseteq \phi_2[c_1/\ex{b}]^{\I}$.\\
     
     % So $|\phi_2[c_1/\ex{b}]^{\I}| = 3 \cdot |V|$.\\ 

     Finally,
     because $(\ex{Vertex} \sqsubseteq \exists \ex{hasColor}) \in \T$,
     each $v \in V^\I$ has a \ex{hasColor}-successor in $\Delta^I$.\\
     Then we have two cases:
     \begin{itemize}
    \item There is a $\ex{w} \in \ex{Vertex}^\I$ and a $\ex{c} \not\in \{\ex{b}, \ex{g},\ex{r}\}$ s.t. $\ex{hasColor}(\ex{w}, \ex{c}) \in \ex{hasColor}^\I$.\\
     % \item There is a $\ex{w} \in \ex{Vertex}^\I$ s.t. $c_{\ex{w}} \notin \{\ex{b, g, r}\}$.
       % Then $|\ex{u}^I| > 3 \cdot |V| + 1$\\
       % Let us focus on the evaluation of $\phi_2$ in $\I$,
       % but restricted to matches that map $c_1$ to \ex{r}.\\
       % Because $\A_3 \subseteq \I$,
       % for every vertex $v \in V$, and for every $c' \in \{\ex{b, g, r}\}$,
       % the mapping $\{v_7 \mapsto v, c_7 \mapsto c'\}$ is an answer to $\phi_2[c_1/\ex{r}]$ in $\I$.\\
       % So $|\phi_2[c_1/\ex{r}]^\I| \geq 3 \cdot |V|$.\\
      Then $\omega = \{v_7 \mapsto \ex{w}, c_7 \mapsto \ex{c}\} \in \phi_2[c_1/\ex{b}]^\I$.\\
      In addition, $\Omega \subseteq \phi_2[c_1/\ex{b}]^\I$ and $\omega \not\in \Omega$.\\
      So $|\phi_2[c_1/\ex{b}]^\I| \geq |\Omega| + 1 = 3 \cdot |V| + 1$.\\
      Therefore $|(\phi_b \wedge \phi_g \wedge \phi_r  \wedge \phi_1  \wedge \phi_2)^\I | \geq 1 \cdot (3 \cdot |V| + 1) = 3 \cdot |V| + 1$.


    \item For each $v \in \ex{Vertex}^\I$, there is a $c \in \{\ex{b}, \ex{g},\ex{r}\}$ s.t. $\ex{hasColor}(v, c) \in \ex{hasColor}^I$.\\
      Because $\G$ is not 3-colorable,
       there must be $\ex{w}_1, \ex{w}_2 \in \ex{Vertex}^I$ and $\ex{c} \in \{\ex{b}, \ex{g},\ex{r}\}$ such that $\ex{edge}(\ex{w}_1, \ex{w}_2) \in \ex{edge}^\I$ and\\
       $\{\ex{hasColor}(\ex{w}_1, \ex{c}),\ex{hasColor}(\ex{w}_2, \ex{c})\} \subseteq \ex{hasColor}^\I$.\\
       \julienbox{
         TODO: double check the following paragraph.
       }
       % So at least one of the following holds:
    %    \[\{
    %    v_1 \mapsto \ex{w}_1,
    %    v_1 \mapsto \ex{w}_2,
    %    c_1 \mapsto \ex{c},
    %    c_2 \mapsto \ex{c}
    %    \} \in \phi_b^\I\],
    %    \[\{
    %    v_3 \mapsto \ex{w}_1,
    %    v_4 \mapsto \ex{w}_2,
    %    c_3 \mapsto \ex{c},
    %    c_4 \mapsto \ex{c}
    %    \} \in \phi_g^\I\]
    %  or
    %    \[\{
    %    v_5 \mapsto \ex{w}_1,
    %    v_6 \mapsto \ex{w}_2,
    %    c_5 \mapsto \ex{c},
    %    c_6 \mapsto \ex{c}
    %    \} \in \phi_r^\I\]

    %    % $\tu \in \phi_b^\I$ or $\tu \in \phi_g^\I$ or $\tu \in \phi_r^\I$.\\
    %  Therefore at least one of
    %  $|\phi_b^\I| \ge 2$,
    %  $|\phi_g^\I| \ge 2$ or
    %  $|\phi_r^\I| \ge 2$
    %  must hold.\\
    %  Since we know that 
    %  $|\phi_b^\I| \ge 1$,
    %  $|\phi_g^\I| \ge 1$, 
    %  $|\phi_r^\I| \ge 1$ and 
    %  $|\phi_0^\I| \geq 3$,
    %  we get:
    %  $$|\phi_0^\I| \cdot |\phi_b^\I| \cdot |\phi_g^\I| \cdot |\phi_r^\I| \ge 3 \cdot 2 \cdot 1 \cdot 1 = 6$$
    %   So there is  a $k_\I > 3$ s.t. $\ans(q,\I) = \{\tup{\varepsilon,k_\I}\}$.
    % \end{itemize}
       
    %  \item For each $v \in \ex{Vertex}^\I$, $c_v \in \{(\ex{b}, \ex{g},\ex{r})\}$.\\
    %    Because $G$ is not 3-colorable,
    %    there must be $v_1, v_2 \in (\ex{Vertex}^I)$ such that $\ex{edge}(v_1, v_2) \in \ex{edge}^\I$ and
    %    $\{\ex{hasColor}(v_1, c_1),\ex{hasColor}(v_2, c_2)\} \subseteq \ex{hasColor}^\I$ for some $c_1, c_2$ such that
    %    \begin{itemize}
    %    \item $c_1, c_2 \in \ex{Red}^\I$, or
    %    \item $c_1, c_2 \in \ex{Blue}^\I$, or
    %    \item $c_1, c_2 \in \ex{Green}^\I$.
    %    \end{itemize}

       Without loss of generality, let $c_1, c_2 \in \ex{Red}^\I$. Then, since for each $v \in \ex{Vertex}^\I$, $c_v \in \{(\ex{b}, \ex{g},\ex{r})\}$, and since $\ex{Red}(\ex{r}) \in \A$, 
       it follows that $|\phi_r^{\I}| \geq 2$ must hold,
       and hence $|\phi_r \wedge \phi_b \wedge \phi_g \wedge \phi_1 \wedge \phi_2|^{\I} \geq 2 \cdot (3 \cdot |V|) = 6 \cdot |V|$.\\
     Therefore $\I \models q_c((), 3 \cdot |V| + 1)$.
     \end{itemize}
     \end{itemize}
    \end{proof}

